On the Power of Threshold-Based Algorithms for Detecting Cycles in the CONGEST Model

It is known that, for every $k\geq 2$, $C_{2k}$-freeness can be decided by a generic Monte-Carlo algorithm running in $n^{1-1/\Theta(k^2)}$ rounds in the CONGEST model. For $2\leq k\leq 5$, faster Monte-Carlo algorithms do exist, running in $O(n^{1-1/k})$ rounds, based on upper bounding the number of messages to be forwarded, and aborting search sub-routines for which this number exceeds certain thresholds. We investigate the possible extension of these threshold-based algorithms, for the detection of larger cycles. We first show that, for every $k\geq 6$, there exists an infinite family of graphs containing a $2k$-cycle for which any threshold-based algorithm fails to detect that cycle. Hence, in particular, neither $C_{12}$-freeness nor $C_{14}$-freeness can be decided by threshold-based algorithms. Nevertheless, we show that $\{C_{12},C_{14}\}$-freeness can still be decided by a threshold-based algorithm, running in $O(n^{1-1/7})= O(n^{0.857\dots})$ rounds, which is faster than using the generic algorithm, which would run in $O(n^{1-1/22})\simeq O(n^{0.954\dots})$ rounds. Moreover, we exhibit an infinite collection of families of cycles such that threshold-based algorithms can decide $\mathcal{F}$-freeness for every $\mathcal{F}$ in this collection.

==> 4-incremental.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Deciding $\mathcal{F}$-Freeness for Incremental Families $\mathcal{F}$}\label{sec_incremental}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section is dedicated to the proof of Theorem~\ref{theo:one-every-four}. In essence, the algorithm deciding $\{C_{4\ell}\mid 1\leq \ell\leq k\}$-freeness performs by successively deciding $C_{4\ell}$-freeness, for $\ell=1,\dots,k$, using threshold-based algorithms. This sequence of algorithms runs in $O(n^{1-1/2k})$ rounds. The same holds for deciding $\{C_{4\ell+2}\mid 1\leq \ell\leq k\}$-freeness, with round-complexity $O(n^{1-1/(2k+1)})$. The proof mostly consists in showing that thresholds can be defined with the guarantee that, if the graph contains a $4\ell$-cycle (or a $(4\ell+2)$-cycle), then this cycle is detected with constant probability. Let us start with $\mathcal{F}_k=\{C_{4\ell}\mid 1\leq \ell\leq k\}$, $k\geq 1$. 

The base case is $\ell=1$, i.e., deciding $C_4$-freeness. It was shown in~\cite{Censor-HillelFG20} that, in this case, a threshold $T_2(1)=1$ suffices.  Let us now assume that we have set up appropriate thresholds for deciding $\mathcal{F}_{k-1}$-freeness. For deciding $\mathcal{F}_k$-freeness, it is sufficient to decide $\mathcal{F}_{k-1}$-freeness first, and then deciding $C_{4k}$-freeness. 
%
Therefore it is sufficient that the algorithm deciding $C_{4k}$-freeness succeeds whenever the graph is $\mathcal{F}_{k-1}$-free. 
%Indeed, if the graph is not $\mathcal{F}_{k-1}$-free, then is it the role of the algorithm checking $\mathcal{F}_{k-1}$-freeness to detect that. 
So, from this point on, we assume that the graph has no $4\ell$-cycles, for all $\ell=1,\dots,k-1$. To decide $C_{4k}$-freeness under this latter hypothesis, we set the thresholds as $T_{2k}(0)=1$, and, for $i\geq 1$, 
\[
T_{2k}(i) = \left\{\begin{array}{ll}
        T_{2k}(i-1) & \mbox{if $i$ is odd,}\\
        (i+1) \cdot T_{2k}(i-1) & \mbox{if $i$ is even.}
    \end{array}\right.
\]


To prove that the thresholds work, let $C=(u_0,\dots,u_{4k-1})$  be a $4k$-cycle in the graph, where $u_0$ is the heavy node with largest degree in~$C$. Let us assume that, for every $i=0,\dots,4k-1$, node~$u_i$ is colored~$i$. Note that this occurs with probability at least $1/(4k+1)^{4k}$. Let $s$ be a neighbor of $u_0$ not belonging to any $4k$-cycle, and let us assume that $s$ is colored~$-1$. We define a well-colored path from $s$ to a node $u_i$ as a path of the form $s,w_0,\dots,w_{i-1},u_i$ where, for every $j=0,\dots,i-1$, node $w_j$ is colored~$j$. The following lemma will also be useful in Section~\ref{section_pairs}.

\begin{lemma}\label{lem-paths-from-single-s}\pierre{move to c12 C14}
Let $i\geq 1$, and let $\rho$ be the maximum number of node-disjoint well-colored paths from $s$ to~$u_i$. If $s$ launches $\textsf{color-BFS}(W)$ from all its heavy neighbors colored~$0$, then $u_i$ cannot receive more than $\rho\cdot T_{2k}(i-1)$ identifiers from nodes colored~$i-1$. 
\end{lemma}

\begin{proof}
Let $S$ be a set of $\rho$ node-disjoint, well-colored paths from $s$ to~$u_i$.
Let $w_0\in W$ be a heavy neighbor of $s$ colored~0, and let us assume that $\id(w_0)$ has reached~$u_i$. It follows that there is a well-colored path~$P$ of length $i$ from $w_0$ to $u_i$. The path~$P$ must intersect some path $P'=\{w'_0,\dots,w'_{i-1}\}$ in~$S$ (perhaps even $P=P'$). As a consequence, $\id(w_0)$ is included in the at most $T_{2p}(i-1)$ identifiers that node $w'_{i-1}$ may forward to~$u_i$. Therefore, the number of identifiers received by $u_i$ during $\textsf{color-BFS}(W)$ does not exceed $\rho\cdot T_{2p}(i-1)$. 
\end{proof}

To prove that our thresholds are sufficient, we now consider separately the odd and even indices. 

\paragraph{Odd indices.} 

The arguments for odd indices are a reformulation of Observation~2 in~\cite{Censor-HillelFG20}, we give them for the sake of completeness.
Let $i$ be an odd index with $1\leq i\leq 2k-1$, and let $\rho$ be the maximum number of node-disjoint, well-colored paths from $s$ to~$u_i$. Let us prove by contradiction that  $\rho=1$ (see Fig.~\ref{fig_incremental}(left) for an illustration of the case $\rho \geq  2$).
Indeed, $\rho\geq 1$ as $\{u_0,\dots,u_{i-1}\}$ is a well-colored path from $s$ to~$u_i$.
Suppose now that there exist two node-disjoint well-colored paths from $s$ to $u_i$, denoted by $P$ and~$P'$. Then $\{s\}\cup P\cup \{u_i\}\cup P'$ is a $(2i+2)$-cycle. As $i$ is odd, we get that $2i+2$ is a multiple of 4. If $i\leq 2k-3$, this contradicts our assumption that the graph is $\mathcal{F}_{k-1}$-free. If $i=2k-1$, then $s$ is in a $4k$-cycle that the algorithm finds when it performs its color-BFS($s$).
Since $\rho=1$, by Lemma~\ref{lem-paths-from-single-s}, node~$u_i$ receives at most $T_{2k}(i-1)$ identifiers.

\paragraph{Even indices.} 

Let $i$ be an even index with $1\leq i \leq 2k-2$, and let $\rho$ be the maximum number of node-disjoint well-colored paths from $s$ to~$u_i$. 
Let us assume that $s$ is such that $u_i$ receives more than $(i+1) \cdot T_{2k}(i-1)$ identifiers from nodes colored~$i-1$. By Lemma~\ref{lem-paths-from-single-s}, $\rho\geq i+2$. Therefore, there exists a well-colored path from $s$ to $u_{i}$ that does not go through $u_0$. Let us denote this path $P=\{w_0,\dots,w_{i-1}\}$.
Let $s'$ be the next node colored $-1$ and neighboring $u_0$ that the algorithm picks. Let us define $\rho'$ as the maximum number of node-disjoint well-colored paths from $s'$ to $u_i$.  If for the source node~$s'$, node $u_i$ also receives more than $(i+1) \cdot T_{2k}(i-1)$ identifiers from nodes colored $i-1$, then, thanks to Lemma~\ref{lem-paths-from-single-s}, $\rho'\geq i+2$. It follows that there exists a well-colored path from $s'$ to $u_i$ that does not go through any of the $i+1$ nodes $u_0, w_0,\dots, w_{i-1}$. Let us denote this path by~$P'$.
As a consequence, $\{s,u_0,s'\}\cup P'\cup \{u_i\} \cup P$ is a $(2i+4)$-cycle (see Fig.~\ref{fig_incremental}(right)). Since $i$ is even, $2i+4$ is a multiple of 4. If $i\leq 2k-4$, this contradicts the assumption that the graph is $\mathcal{F}_{k-1}$-free. If $i=2k-2$, then $s$ is in a $4k$-cycle, which is detected by~$s$.
Therefore, if the algorithm picks a neighbor $s$ of $u_0$ colored $-1$ that causes $u_i$ to receive more than $T_{2k}(i)$ identifiers, then no other neighbor $s'$ of $u_0$ can also cause $u_i$ to receive more than $T_{2k}(i)$ identifiers, as $s$ would then be in a cycle would be detected by~$s$.

\begin{figure}
\centering
\includegraphics[scale=0.75]{figures/incremental.pdf}
\caption{Cycles of $\mathcal{F}_{k-1}$ or a $4k$-cycle appearing if neighbors of $u_0$ have several paths to $u_i$. On the left, $i$ is odd, on the right it is even.}
\label{fig_incremental}
\end{figure}

\paragraph{Wrap up.}

It results from our analyses for odd and even indices that at most  $k-1$ neighbors $s$ of $u_0$ colored $-1$ may prevent the detection of the $4k$-cycle $(u_0,\dots,u_{4k-1})$, namely at most one source~$s$ for each node $u_{2i}$, for $1\leq i\leq k-1$. Since there are $\Omega(n^{1/2k})$ neighbors of $u_0$ colored~$-1$, the algorithm will  randomly choose at least $k$ different neighbors of~$u_0$ whenever $O(n^{1-1/2k})$ random choices are performed. This completes the proof for $\{C_{4\ell}\mid 1\leq \ell\leq k\}$-freeness, $k\geq 1$. 

\paragraph{$\{C_{4\ell+2}\mid 1\leq \ell \leq k\}$-freeness.}

\mael{Nouveau: a lire} The proof for $\{C_{4l}|2\leq l\leq p\}$-freeness can be adapted with very little changes to $\{C_{4l+2}|2\leq l\leq p\}$-freeness by inverting the roles of odd and even values of $i$ to compute $T_{2p+1}(i)$.

Indeed, let $i$ be an even index. Similarly to the case of odd indices for $\{C_{4l}|2\leq l\leq p\}$-freeness, if there are two node-disjoint well-colored paths from a picked $s$ to $u_i$, then $s$ is in a $(2i+2)$-cycle (see Fig.~\ref{fig_incremental}(left)). With $i$ being even, the cycle belongs to $\{C_{4l+2}|2\leq l\leq p\}$.

On the other hand, let $i$ be an odd index. Similarly to the case of even indices for $\{C_{4l}|2\leq l\leq p\}$-freeness, if $u_i$ receives more than $(i+1)T_{2k}(i-1)$ identifiers for two different picked nodes $s$ and $s'$, then $s$ is in a $(2i+4)$-cycle (see Fig.~\ref{fig_incremental}(right)). With $i$ being odd, the cycle belongs to $\{C_{4l+2}|2\leq l\leq p\}$.

Consequently, the algorithm works by fixing $T_{2k}(0)=1$ and, for $i\geq 1$, 
\[
T_{2k}(i) = \left\{\begin{array}{ll}
        (i+1) \cdot T_{2k}(i-1) & \mbox{if $i$ is odd,}\\
         T_{2k}(i-1) & \mbox{if $i$ is even.}
    \end{array}\right.
\]

